A Majorization-Minimization with Monte Carlo Approach for Hyperparameter Estimation

We consider inverse problems with linear forward models and Gaussian priors, but with unknown hyperparameters that may arise from the model, the noise, or the specification of the prior. We model this using a hierarchical Bayes framework resulting in a posterior distribution that is non-Gaussian, in general, and challenging to sample from. Consequently, we use an empirical Bayes framework for estimating the maximum a posteriori estimate of the hyperpameters by considering the marginalized posterior distribution. However, the optimization problem is also computationally challenging due to the need for repeated evaluation of log determinants. To address this issue, we propose a Majorization-Minimization with Monte Carlo approach, which we call M$^{3}$C, for hyperparameter estimation. Specifically, we replace the challenging optimization problem with a sequence of simpler ones by utilizing a majorization function (or majorant) for the log-determinant term, combined with a Monte Carlo estimator to approximate the majorant. We provide theoretical results, showing that under certain assumptions, the M$^{3}$C iterates converge with high probability to a critical point of the original cost function. A variety of numerical examples are provided from seismic tomography, super-resolution imaging, and contaminant source identification.

==> SRresults/64x64Results.tex <==
\begin{figure}
    \centering
\begin{tabular}{|c|cccc|}
     \hline
     % 64x64
     \multicolumn{5}{|c|}{$64\times64$}\\ \hline
     True & \multicolumn{4}{c|}{Low Resolution Images}  \\
     \includegraphics[width=.165\textwidth]{SRresults/ref/SR_n64_true.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR1_SR_n64_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR3_SR_n64_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR5_SR_n64_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR7_SR_n64_k8.png} \\ 
     Reference & \multicolumn{4}{c|}{} \\
     \includegraphics[width=.165\textwidth]{SRresults/ref/Ref_SR_n64_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR2_SR_n64_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR4_SR_n64_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR6_SR_n64_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR8_SR_n64_k8.png} \\ \hline \hline
     % 128x128
     \multicolumn{5}{|c|}{$128\times128$}\\ \hline
     True & \multicolumn{4}{c|}{Low Resolution Images}  \\
     \includegraphics[width=.165\textwidth]{SRresults/ref/SR_n128_true.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR1_SR_n128_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR3_SR_n128_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR5_SR_n128_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR7_SR_n128_k8.png} \\ 
     Reference & \multicolumn{4}{c|}{} \\
     \includegraphics[width=.165\textwidth]{SRresults/ref/Ref_SR_n128_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR2_SR_n128_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR4_SR_n128_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR6_SR_n128_k8.png}
     & \includegraphics[width=.165\textwidth]{SRresults/ref/LR8_SR_n128_k8.png} \\ \hline
     
     
\end{tabular}
    \caption{True high resolution image and reference images}
    \label{fig:SR_ref}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{|c| c c | c c |}
     \hline
     \multicolumn{5}{|c|}{SAA} \\ \hline \hline
     % 64x64
     \multicolumn{5}{|c|}{$64\times 64$} \\ \hline
     \multicolumn{5}{|c|}{$\lambda=20$ and $\sigma=0.12$} \\ \hline
     $\bfy_t$ & \multicolumn{2}{c|}{$\bfy_0$} & \multicolumn{2}{c|}{$\bfy_f$} \\ 
     \includegraphics[width=.175\textwidth]{SRresults/SR/SRresults_yt_n64.png}
     & \includegraphics[width=.175\textwidth]{SRresults/SR/SRresults_y0_n64.png}
     & \includegraphics[width=.145\textwidth]{SRresults/SR/params_y0_SR_n64.png} 
     & \includegraphics[width=.175\textwidth]{SRresults/SR/SRresults_yf_n64.png}
     & \includegraphics[width=.145\textwidth]{SRresults/SR/params_yf_SR_n64.png} 
     \\ \hline \hline
     
     % 128x128
     \multicolumn{5}{|c|}{$128\times 128$} \\ \hline
     \multicolumn{5}{|c|}{$\lambda=25$ and $\sigma=0.13$} \\ \hline
     $\bfy_t$ & \multicolumn{2}{c|}{$\bfy_0$} & \multicolumn{2}{c|}{$\bfy_f$} \\ 
     \includegraphics[width=.175\textwidth]{SRresults/SR/SRresults_yt_n128.png}
     & \includegraphics[width=.175\textwidth]{SRresults/SR/SRresults_y0_n128.png}
     & \includegraphics[width=.145\textwidth]{SRresults/SR/params_y0_SR_n128.png} 
     & \includegraphics[width=.175\textwidth]{SRresults/SR/SRresults_yf_n128.png}
     & \includegraphics[width=.145\textwidth]{SRresults/SR/params_yf_SR_n128.png} \\ \hline
\end{tabular}
\caption{SR $64\times 64$ and $128\times 128$ reconstructions and parameters at $\bfy_t$, $\bfy_0$, and $\bfy_f$ using SAA.}
\label{fig:SR_recon}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{|c c c|}
    \hline
    \multicolumn{3}{|c|}{MM-SAA} 
    \\ \hline \hline
    \multicolumn{3}{|c|}{$64\times64$: $\lambda=20$ and $\sigma=0.12$} 
    \\ \hline
    $\bfy_t$ &  \multicolumn{2}{c|}{$\bfy_0$} 
    \\
    \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_yt_n64_k8.png}
    & \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_y0_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/SR/params_y0_SR_n64_k8.png} 
    \\ \hline
    Maximum & \multicolumn{2}{c|}{$\bfy_f$} \\
    Inner Iteration & &
    \\
    2 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/2/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/2/params_yf_SR_n64_k8.png}
    \\
    50 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/50/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/50/params_yf_SR_n64_k8.png}
    \\
    100 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/100/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/100/params_yf_SR_n64_k8.png}
    \\
    150 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/150/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/150/params_yf_SR_n64_k8.png}
    \\
    200 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/300/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/300/params_yf_SR_n64_k8.png}
    \\ \hline
\end{tabular}
\caption{SR $64\times 64$ reconstructions and parameters at $\bfy_t$, $\bfy_0$, and $\bfy_f$ for MM approach using varying maximum inner iterations.}
%\label{fig:placeholder}
\end{figure}

\begin{figure}
\begin{minipage}{.67\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|}
    \cline{2-5}
    \multicolumn{1}{c|}{} & \multicolumn{4}{c|}{SAA} \\ \cline{2-5} 
    \multicolumn{1}{c|}{} & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} & Rel. \\ 
    \multicolumn{1}{c|}{} & Iter. & Evals. & & Error \\ \cline{2-5}
    \multicolumn{1}{c|}{} & 72 & 308 & 825 & 0.223 \\
    \cline{2-5} 
    \multicolumn{5}{c}{} \\
    \hline
    % \multicolumn{5}{|c|}{MM-SAA} \\ \hline
    % Maximum & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} & Rel. \\
    % Inner Iter. & Iter. & Evals. & & Error \\ \hline
    % 2 & 619 & 5,529 & $9.65 \times 10^3$ &\\
    % 50 & 215 & 1,005 & $1.81 \times 10^3$ &\\
    % 100 & 207 & 946 & $1.72\times 10^3$& \\
    % 150 & 212 & 973 & $1.76\times 10^3$& \\
    % 200 & 246 & 1,104 & $1.99\times 10^3$ &\\ \hline
    % \multicolumn{5}{|c|}{MM-SAA (Projected Gradient)} \\ \hline
    % Maximum & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} & Rel. \\
    % Inner Iter. & Iter. & Evals. & & Error \\ \hline
    % 50 & 668 & & $1.93\times 10^3$ & \\
    % 100 & 680 & & $2.61\times 10^3$ & \\
    % 150 & 714 & & $3.53\times 10^3$ & 
    % \\ \hline 
    % \multicolumn{5}{c}{} \\
    % \hline
    \multicolumn{5}{|c|}{MM-SAA (Projected Gradient w/ Finite Diff.)} \\ \hline
    Maximum & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} & Rel. \\
    Inner Iter. & Iter. & Evals. & & Error \\ \hline
    50 & 56 & & 37 & 0.217 \\
    100 & 349 & & 217 & 0.222 \\
    150 & 1,035 & & 638 & 0.216
    \\ \hline
\end{tabular}
\captionof{table}{Total iterations, function evaluations, and runtime for SAA and MM approach in the $64\times 64$ super resolution problem. The relative error of the reconstruction at $\bfy_t$ is 0.19.}
\end{minipage}
\hfill
\begin{minipage}{.28\textwidth}
\centering
\includegraphics[width=1\textwidth]{SRresults/FD/SR_mmIterAll_n64.png}
\captionof{figure}{Number of inner iterations completed at each outer iteration for various maximum inner iterations for the $64\times 64$ super resolution problem.}
\end{minipage}
\end{figure}

%%%%%% proj grad dec
\begin{figure}
\centering
\begin{tabular}{|c c c|}
    \hline
    \multicolumn{3}{|c|}{MM-SAA: Projected Gradient} 
    \\ \hline \hline
    \multicolumn{3}{|c|}{$64\times64$: $\lambda=20$ and $\sigma=0.12$} 
    \\ \hline
    $\bfy_t$ &  \multicolumn{2}{c|}{$\bfy_0$} 
    \\
    \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_yt_n64_k8.png}
    & \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_y0_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/SR/params_y0_SR_n64_k8.png} 
    \\ \hline
    Maximum & \multicolumn{2}{c|}{$\bfy_f$} \\
    Inner Iteration & &
    \\
    % 2 
    % & \includegraphics[width=.20\textwidth]{SRresults/PGD/2/SRresults_yf_n64_k8.png} 
    % & \includegraphics[width=.17\textwidth]{SRresults/PGD/2/params_yf_SR_n64_k8.png}
    % \\
    50 
    & \includegraphics[width=.20\textwidth]{SRresults/PGD/50/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/PGD/50/params_yf_SR_n64_k8.png}
    \\
    100 
    & \includegraphics[width=.20\textwidth]{SRresults/PGD/100/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/PGD/100/params_yf_SR_n64_k8.png}
    \\
    150 
    & \includegraphics[width=.20\textwidth]{SRresults/PGD/150/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/PGD/150/params_yf_SR_n64_k8.png}
    \\ \hline
\end{tabular}
\caption{SR $64\times 64$ reconstructions and parameters at $\bfy_t$, $\bfy_0$, and $\bfy_f$ for MM approach with projected gradient using varying maximum inner iterations.}
%\label{fig:placeholder}
\end{figure}

%%%%%% proj grad dec with finite difference
\begin{figure}
\centering
\begin{tabular}{|c c c|}
    \hline
    \multicolumn{3}{|c|}{MM-SAA: Projected Gradient with Finite Difference} 
    \\ \hline \hline
    \multicolumn{3}{|c|}{$64\times64$: $\lambda=20$ and $\sigma=0.12$} 
    \\ \hline
    $\bfy_t$ &  \multicolumn{2}{c|}{$\bfy_0$} 
    \\
    \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_yt_n64_k8.png}
    & \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_y0_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/SR/params_y0_SR_n64_k8.png} 
    \\ \hline
    Maximum & \multicolumn{2}{c|}{$\bfy_f$} \\
    Inner Iteration & &
    \\
    % 2 
    % & \includegraphics[width=.20\textwidth]{SRresults/FD/2/SRresults_yf_n64_k8.png} 
    % & \includegraphics[width=.17\textwidth]{SRresults/FD/2/params_yf_SR_n64_k8.png}
    % \\
    50 
    & \includegraphics[width=.20\textwidth]{SRresults/FD/50/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/FD/50/params_yf_SR_n64_k8.png}
    \\
    100 
    & \includegraphics[width=.20\textwidth]{SRresults/FD/100/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/FD/100/params_yf_SR_n64_k8.png}
    \\
    150 
    & \includegraphics[width=.20\textwidth]{SRresults/FD/150/SRresults_yf_n64_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/FD/150/params_yf_SR_n64_k8.png}
    
    \\ \hline
\end{tabular}
\caption{SR $64\times 64$ reconstructions and parameters at $\bfy_t$, $\bfy_0$, and $\bfy_f$ for MM approach with projected gradient using varying maximum inner iterations.}
%\label{fig:placeholder}
\end{figure}

==> abbrev.tex <==

%\usepackage{authblk}
\usepackage{setspace}
%\usepackage{bbold}
\usepackage{makecell}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{subcaption}
%\RequirePackage{amsmath, amsthm}
% \RequirePackage{alltt, moreverb}           % improve verbatim
% \RequirePackage{showkeys, showidx}         % print labels, etc. in draft-mode (fold)
%\RequirePackage{graphicx}
% \RequirePackage[utf8]{inputenc}            % write with Umlaute (fold)

% \RequirePackage{algorithm}
%\RequirePackage{algpseudocode}
% \RequirePackage{colortbl}
\RequirePackage{multirow}
\RequirePackage{adjustbox}
%\RequirePackage{algorithmicx}
\RequirePackage{colortbl}
\RequirePackage{import}
\RequirePackage{hyperref}
\RequirePackage{stackrel}
\RequirePackage{wrapfig}
\RequirePackage{xspace} % create space or not after defined word
% \RequirePackage{shellesc}
\RequirePackage{bm}
\usepackage{cleveref}

\newcommand{\normtwo}[1]{\|#1\|_2}
\newcommand{\krylov}[1]{\mathcal{K}_{#1}}
\newcommand{\mb}[1]{\mathbb{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\B}[1]{\boldsymbol{#1}}
\newcommand{\post}{\boldsymbol\Gamma_\text{\rm post}}
\newcommand{\postmu}{\boldsymbol\mu_\text{\rm post}}
\newcommand{\Span}[1]{\text{Span}\left\{#1\right\}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\posth}{\widehat{\boldsymbol{\Gamma}}_\text{\rm post}}
\newcommand{\xpost}{{\bfx}_\text{post}}
\newcommand{\xsamp}{\bfx^\star}
\newcommand{\ysamp}{\bfy^\star}
\newcommand{\zsamp}{\bfz^\star}
\newcommand{\xmap}{\bfx_{\rm MAP}}
\newcommand{\zmap}{\bfz_{\rm MAP}}
\newcommand{\ymap}{\bfy_{\rm MAP}}
\newcommand{\zmean}{\hat{\bfz}}
\newcommand{\xmean}{\hat{\bfx}}
\newcommand{\ymean}{\hat{\bfy}}
\newcommand{\sposth}{\widehat{\bfs}_\text{post}}
\newcommand{\gammah}{\widehat{\boldsymbol{\Gamma}}}
\newcommand{\fhat}{\hat{f}(\bfz)}
\newcommand{\fhaty}{\hat{f}_y(\bfy)}

\newcommand{\eps} {\varepsilon}                            % redefine epsilon
\newcommand{\mdot} {\,\cdot\,}
\newcommand{\D}   {{\rm D}}                                % differential D
\newcommand{\F}   {{\rm F}}                  
\newcommand{\fro}   {{\rm F}} % differential D
\newcommand{\tol} {{\rm tol}}                              % tolerance
\newcommand{\e}   {\textnormal{e}}                         % Eulerian number
\newcommand{\clos}{\textnormal{Closure}}                   % closure
\newcommand{\im}  {\textnormal{Im }}                       % imaginary part
\newcommand{\re}  {\textnormal{Re }}                       % real part
\newcommand{\hf}  {\frac{1}{2}}                            % 1/2
\newcommand{\thf}  {\tfrac{1}{2}}                            % 1/2
\DeclareMathOperator*{\argmin}{arg\,min}                   % arg min
\DeclareMathOperator*{\argmax}{arg\,max}                   % arg max
\renewcommand{\i} {\textnormal{i}}                         % imaginary unity
\renewcommand{\t} {^{\top}}                                % transpose, e.g. $A\t$
\renewcommand{\d} {{\rm d}}                                % differential d
\renewcommand{\H} {^{{\rm H}}}                             % Hermitian
\renewcommand{\vec}[1] {{\rm vec}(#1)}                     % vectorize matrix
\newcommand{\inner} [2]{\langle #1,#2\rangle}           % f.e. \inner product[\infty]{A-B}
\newcommand{\norm} [2][]{\left\|#2\right\|_{#1}}           % f.e. \norm[\infty]{A-B}
\newcommand{\abs}  [2][]{\left|#2\right|_{#1}}             % f.e. \abs[\infty]{A-B}
\newcommand{\cond} [2][]{{\rm cond}_{#1}\left( #2 \right)} % f.e. \cond[\infty]{A}
\newcommand{\pow}  [1]  {^{\left(#1\right)}}               % brackets exponent
\newcommand{\sign} [1]  {{\rm sign\!}\left( #1 \right)}    % signum
\newcommand{\rank} [1]  {{\rm rank\!}\left( #1 \right)}    % rank of a matrix
%\newcommand{\diag} [1]  {{\rm diag\!}\left( #1 \right)}    % diagonal of a matrix
\newcommand{\spann}[1]  {{\rm span\!}\left( #1 \right)}    % span of a function % Careful \span conflicts with amsmath!!!!!!!!!!
\newcommand{\range}[1]  {{\rm range\!}\left( #1 \right)}    % span of a function
\renewcommand{\ker}[1]  {{\rm ker\!}\left( #1 \right)}     % kernel of a function
\newcommand{\ul}   [1]  {\underline{#1}}                   % shorted underline
% \newcommand{\email}[1]  {\texttt{#1}}                      % email
\newcommand{\kron}{\otimes}                                % Kronecker product
% \newcommand{\trace} [1]  {{\rm trace\!}\left( #1 \right)}  % trace of a matrix
%\newcommand{\trace} [1]  {{\rm tr\!}\left( #1 \right)}
\newcommand{\trace}{\mathsf{trace}}% trace of a matrix
% \newcommand{\acknowledgement}[1]{\noindent\textbf{Acknowledgement: }#1}   % acknowledgement
% \newcommand\figurescale{1}
\newcommand{\bfxh}{\widehat\bfx}
\newcommand{\exact} {{\rm exact}}     

\newcommand{\logdet}{\mathsf{logdet}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}
\renewcommand{\log}{\mathsf{log}}% exact
\renewcommand{\det}{\mathsf{det}}
\newcommand{\diag}{\mathsf{diag}}

\newcommand{\Var}{\mathbb{V}\mathrm{ar}}
\newcommand{\Cov}{\mathbb{C}\mathrm{ov}}
\newcommand{\iid}{iid}
\newcommand{\bigO}  [1]  {\calO\!\left(#1\right)}
% \newcommand{\tia}[1] {{\color{orange} #1}}
% \newcommand{\eric}[1]{{\color{maroon} #1}}
% small o-notation
\newcommand\calo{
  \mathchoice
    {{\scriptstyle\mathcal{O}}}% \displaystyle
    {{\scriptstyle\mathcal{O}}}% \textstyle
    {{\scriptscriptstyle\mathcal{O}}}% \scriptstyle
    {\scalebox{.7}{$\scriptscriptstyle\mathcal{O}$}}%\scriptscriptstyle
  }


  % <fold> bold letters and numbers with \bf
\newcommand{\p}{{\rm p}}                     % probability density

\newcommand{\bfGamma}{{\boldsymbol{\Gamma}}}
\newcommand{\bfDelta}{{\boldsymbol{\Delta}}}
\newcommand{\bfTheta}{{\boldsymbol{\Theta}}}
\newcommand{\bfLambda}{{\boldsymbol{\Lambda}}}
\newcommand{\bfXi}{{\boldsymbol{\Xi}}}
\newcommand{\bfPi}{{\boldsymbol{\Pi}}}
\newcommand{\bfSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bfUpsilon}{{\boldsymbol{\Upsilon}}}
\newcommand{\bfPhi}{{\boldsymbol{\Phi}}}
\newcommand{\bfPsi}{{\boldsymbol{\Psi}}}
\newcommand{\bfOmega}{{\boldsymbol{\Omega}}}
\newcommand{\bfalpha}{{\boldsymbol{\alpha}}}
\newcommand{\bfbeta}{{\boldsymbol{\beta}}}
\newcommand{\bfgamma}{{\boldsymbol{\gamma}}}
\newcommand{\bfdelta}{{\boldsymbol{\delta}}}
\newcommand{\bfepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\bfvarepsilon}{{\boldsymbol{\varepsilon}}}
\newcommand{\bfeps}{{\boldsymbol{\varepsilon}}}
\newcommand{\bfzeta}{{\boldsymbol{\zeta}}}
\newcommand{\bfeta}{{\boldsymbol{\eta}}}
\newcommand{\bftheta}{{\boldsymbol{\theta}}}
\newcommand{\bfvartheta}{{\boldsymbol{\theta}}}
\newcommand{\bfiota}{{\boldsymbol{\iota}}}
\newcommand{\bfkappa}{{\boldsymbol{\kappa}}}
\newcommand{\bflambda}{{\boldsymbol{\lambda}}}
\newcommand{\bfmu}{{\boldsymbol{\mu}}}
\newcommand{\bfnu}{{\boldsymbol{\nu}}}
\newcommand{\bfxi}{{\boldsymbol{\xi}}}
\newcommand{\bfo}{{\boldsymbol{o}}}
\newcommand{\bfpi}{{\boldsymbol{\pi}}}
\newcommand{\bfvarpi}{{\boldsymbol{\varpi}}}
\newcommand{\bfrho}{{\boldsymbol{\rho}}}
\newcommand{\bfvarrho}{{\boldsymbol{\varrho}}}
\newcommand{\bfsigma}{{\boldsymbol{\sigma}}}
\newcommand{\bfvarsigma}{{\boldsymbol{\varsigma}}}
\newcommand{\bftau}{{\boldsymbol{\tau}}}
\newcommand{\bfupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\bfphi}{{\boldsymbol{\phi}}}
\newcommand{\bfvarphi}{{\boldsymbol{\varphi}}}
\newcommand{\bfchi}{{\boldsymbol{\chi}}}
\newcommand{\bfpsi}{{\boldsymbol{\psi}}}
\newcommand{\bfomega}{{\boldsymbol{\omega}}}

\newcommand{\bfA}{{\bf A}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfC}{{\bf C}}
\newcommand{\bfD}{{\bf D}}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfF}{{\bf F}}
\newcommand{\bfG}{{\bf G}}
\newcommand{\bfH}{{\bf H}}
\newcommand{\bfI}{{\bf I}}
\newcommand{\bfJ}{{\bf J}}
\newcommand{\bfK}{{\bf K}}
\newcommand{\bfL}{{\bf L}}
\newcommand{\bfM}{{\bf M}}
\newcommand{\bfN}{{\bf N}}
\newcommand{\bfO}{{\bf O}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfR}{{\bf R}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfT}{{\bf T}}
\newcommand{\bfU}{{\bf U}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfZ}{{\bf Z}}
\newcommand{\bfa}{{\bf a}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfh}{{\bf h}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfl}{{\bf l}}
\newcommand{\bfm}{{\bf m}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bft}{{\bf t}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfz}{{\bf z}}


\newcommand{\bfzero}{{\bf0}}
\newcommand{\bfone}{{\bf1}}
\newcommand{\bftwo}{{\bf2}}
\newcommand{\bfthree}{{\bf3}}
\newcommand{\bffour}{{\bf4}}
\newcommand{\bffive}{{\bf5}}
\newcommand{\bfsix}{{\bf6}}
\newcommand{\bfseven}{{\bf7}}
\newcommand{\bfeight}{{\bf8}}
\newcommand{\bfnine}{{\bf9}}
% </fold>

% <fold> bold letters with \mx
\newcommand{\mxA}{{\bf A}}
\newcommand{\mxB}{{\bf B}}
\newcommand{\mxC}{{\bf C}}
\newcommand{\mxD}{{\bf D}}
\newcommand{\mxE}{{\bf E}}
\newcommand{\mxF}{{\bf F}}
\newcommand{\mxG}{{\bf G}}
\newcommand{\mxH}{{\bf H}}
\newcommand{\mxI}{{\bf I}}
\newcommand{\mxJ}{{\bf J}}
\newcommand{\mxK}{{\bf K}}
\newcommand{\mxL}{{\bf L}}
\newcommand{\mxM}{{\bf M}}
\newcommand{\mxN}{{\bf N}}
\newcommand{\mxO}{{\bf O}}
\newcommand{\mxP}{{\bf P}}
\newcommand{\mxQ}{{\bf Q}}
\newcommand{\mxR}{{\bf R}}
\newcommand{\mxS}{{\bf S}}
\newcommand{\mxT}{{\bf T}}
\newcommand{\mxU}{{\bf U}}
\newcommand{\mxV}{{\bf V}}
\newcommand{\mxW}{{\bf W}}
\newcommand{\mxX}{{\bf X}}
\newcommand{\mxY}{{\bf Y}}
\newcommand{\mxZ}{{\bf Z}}
\newcommand{\mxSigma}{{\bf \Sigma}}
% </fold>

% <fold> calligraphic characters
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}
% </fold>

% <fold> blackboard characters
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}
% </fold>

% <fold> mathematical fracture characters (requires amsmath)
\newcommand{\mfA}{\mathfrak{A}}
\newcommand{\mfB}{\mathfrak{B}}
\newcommand{\mfC}{\mathfrak{C}}
\newcommand{\mfD}{\mathfrak{D}}
\newcommand{\mfE}{\mathfrak{E}}
\newcommand{\mfF}{\mathfrak{F}}
\newcommand{\mfG}{\mathfrak{G}}
\newcommand{\mfH}{\mathfrak{H}}
\newcommand{\mfI}{\mathfrak{I}}
\newcommand{\mfJ}{\mathfrak{J}}
\newcommand{\mfK}{\mathfrak{K}}
\newcommand{\mfL}{\mathfrak{L}}
\newcommand{\mfM}{\mathfrak{M}}
\newcommand{\mfN}{\mathfrak{N}}
\newcommand{\mfO}{\mathfrak{O}}
\newcommand{\mfP}{\mathfrak{P}}
\newcommand{\mfQ}{\mathfrak{Q}}
\newcommand{\mfR}{\mathfrak{R}}
\newcommand{\mfS}{\mathfrak{S}}
\newcommand{\mfT}{\mathfrak{T}}
\newcommand{\mfU}{\mathfrak{U}}
\newcommand{\mfV}{\mathfrak{V}}
\newcommand{\mfW}{\mathfrak{W}}
\newcommand{\mfX}{\mathfrak{X}}
\newcommand{\mfY}{\mathfrak{Y}}
\newcommand{\mfZ}{\mathfrak{Z}}
\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}


\newcommand{\defeq}{\mathrel{\overset{\makebox[0pt]{\text{\tiny def}}}{=}}}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\myP}{\mathbb{P}}
\DeclareMathOperator{\Ey}{\mathbb{E}_{\epsilon}}
\DeclareMathOperator{\Ew}{\mathbb{E}_{\vw}}
\DeclareMathOperator{\Es}{\mathbb{E}_{\vs}}
\DeclareMathOperator{\V}{\mathbb{V}\mathrm{ar}}

% For comments
\newcommand{\hugo}[1]{\textcolor{teal}{[Hugo: #1]}}

\usepackage{mathtools}

\makeatletter
\DeclareRobustCommand\widecheck[1]{{\mathpalette\@widecheck{#1}}}
\def\@widecheck#1#2{%
    \setbox\z@\hbox{\m@th$#1#2$}%
    \setbox\tw@\hbox{\m@th$#1%
       \widehat{%
          \vrule\@width\z@\@height\ht\z@
          \vrule\@height\z@\@width\wd\z@}$}%
    \dp\tw@-\ht\z@
    \@tempdima\ht\z@ \advance\@tempdima2\ht\tw@ \divide\@tempdima\thr@@
    \setbox\tw@\hbox{%
       \raise\@tempdima\hbox{\scalebox{1}[-1]{\lower\@tempdima\box
\tw@}}}%
    {\ooalign{\box\tw@ \cr \box\z@}}}
\makeatother


==> blinddeconv.tex <==
\subsection{Blind Image Deconvolution} 
\label{sec:bd}
Next, we consider a blind deconvolution problem where $\bfb$ is a blurred and noisy image, and $\bfx$ is the target image we hope to recover. The matrix $\bfA(\bfy)$ models the blurring operation which can be written as 
$$ \bfA(\bfy) = \bfA(\bfP(\bfy))$$
where $\bfP(\bfy)$ is a point spread function (PSF). Let $\bftheta = [\lambda,\sigma]\t$ such that $\bfx\mid\bftheta\sim \mc{N}(\bfmu_x,\lambda\bfQ_x)$ and $\bfe\mid\bftheta\sim \mc{N}(\bf0,\sigma\bfR)$.
%In this problem, we assume a Gaussian blur where the PSF, centered at $k,l$, has the form...

%Here $s_1$, $s_2$, and $r$ are unknown parameters that determine the spread and orientation of the PSF. 
%Let $$\bfy = \begin{bmatrix} s_1 \\ s_2 \\ r \end{bmatrix}$$
We assume a Gaussian blur where the PSF, centered at $(k,l)$, has the form
\begin{align}
    p_{ij} &= \exp\left( -\frac{1}{2}\begin{bmatrix} i-k \\ j-l \end{bmatrix}\t \underbrace{\begin{bmatrix} l_1 & 0 \\ l_2 & l_3 \end{bmatrix}\begin{bmatrix} l_1 & l_2 \\ 0 & l_3 \end{bmatrix}}_{=\bfL\bfL\t} \begin{bmatrix} i-k \\ j-l \end{bmatrix}\right)  \label{eq:PSF} \\
    &= \exp\left( \big( (i-k)l_1 + (j-l)l_2 \big)^2 + l_3^2(j-l)^2 \right) \notag
\end{align}
% \begin{align*}
%     p_{ij} &= \exp\left( -\frac{1}{2}\begin{bmatrix} i-k \\ j-l \end{bmatrix}\t \begin{bmatrix} s_1^2 & 0 \\ 0 & s_2^2 \end{bmatrix}^{-1} \begin{bmatrix} i-k \\ j-l \end{bmatrix}\right) \\
%     &= \exp\left(-\frac{(i-k)^2}{2s_1^2}-\frac{(j-l)^2}{2s_2^2}\right)
% `\end{align*}
where $\bfL\bfL\t$ is a Cholesky factorization of a matrix whose entries are determined by the spread and rotation of the PSF. Let
\begin{equation*}
    \bfy = \begin{bmatrix}
        l_1 \\ l_2 \\ l_3
    \end{bmatrix}
\end{equation*}
and $\bfA(\bfy)$ be the Gaussian PSF with parameters $\bfy$.

We consider a small example where $\bfx$ and $\bfb$ are vectorized $32\times32$ images so the full objective function in \eqref{eq:fullopt} can be computed exactly for comparison. The hyperparameters are fixed to be $\lambda=1/200$, $\sigma = 5.55\times 10^{-6}$ and we assume $\bfmu_y = \bf1$, $\bfQ_y = \bfI$, $\bfmu_x = \bf0$ and $\bfQ_x=\bfI$.  

To visualize the objective function, let $l_2=0$ and $\bfy_{t} = [.5^{-1/2},1]\t$ be the true model parameters. Now $\bfy = [l_1, l_2]\t$ are the unknowns, and Figure \ref{fig:objFun_l} shows the full objective function and its individual terms. Additionally, by fixing $l_2 = 1$, we can visualize the surrogate function $\mc{G}(l_1\mid y_k)$. In Figure \ref{fig:BGmaj}, a plot of $\mc{G}(l_1\mid 1.2)$ (i.e. the majorization around the point $y_k = 1.2$) is shown in comparison with the full objective function $\mc{F}(l_1)$.

\begin{figure}
\centering
\begin{tabular}{cc|ccc}
    \multirow{2}{*}{True} & \multirow{2}{*}{Observed} & \multicolumn{3}{c}{Reconstructions} \\
    & & $\bfy_t$ & $\bfy_0$ & $\bfy_f$ \\
    \includegraphics[width=.165\textwidth]{BDresults/BD_true_n32.png} & 
    \includegraphics[width=.165\textwidth]{BDresults/BD_blur_n32.png} & 
    \includegraphics[width=.165\textwidth]{BDresults/BDFresults_yt_n32_Ireg_l.png} & 
    \includegraphics[width=.165\textwidth]{BDresults/BDFresults_y0_n32_Ireg_l.png} & 
    \includegraphics[width=.165\textwidth]{BDresults/BDFresults_yf_n32_Ireg_l.png}
    
\end{tabular}
\caption{The true and observed images and reconstructions at $\bfy_t$, $\bfy_0$, and $\bfy_f$ for the two parameter blind deconvolution setup.}
\label{fig:BD_im}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{BDresults/MM/majorFn_l1.png}
    \caption{The majorization, $\mc{G}(l_1\mid y_k)$, of $\mc{F}(l_1)$ around the point $y_k=1.2$ with fixed $l_2=1$ for the blind deconvolution problem. }
    \label{fig:BDmaj}
\end{figure}

\begin{figure}
    \centering
    \begin{tabular}{cccc}
        $\scriptstyle\mc{F}(\bfy)$ & $\scriptstyle\frac12\logdet\Psi(\bfy)$ & $\scriptstyle\frac12 \|\bfA(\bfy) \bfmu_x - \bfb\|_{\bfPsi(\bfy)^{-1}}^2$ &  $\scriptstyle-\log\pi_{y}(\bfy)$ \\
        \includegraphics[width=.215\textwidth]{BDresults/BD_full_objfn_32_Ireg_l.png} &
        \includegraphics[width=.215\textwidth]{BDresults/BD_full_objfnF1_32_Ireg_l.png} &
        \includegraphics[width=.215\textwidth]{BDresults/BD_full_objfnF2_32_Ireg_l.png} &
        \includegraphics[width=.215\textwidth]{BDresults/BD_full_objfnF3_32_Ireg_l.png}
    \end{tabular}
        \caption{Full objective function over the grid $[0.25,2.5]\times [0.25,2.5]$.}
        \label{fig:objFun_l}
\end{figure}

\begin{figure}[ht!]
    \centering
    \begin{subfigure}{.24\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/SAA/BD_objfn_opt_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.44\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/SAA/params_BD_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.22\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/SAA/BDFresults_yf_n32.png}
    \end{subfigure}
    \caption{SAA: Optimization iteration history visualized on the objective function (left), as individual parameters compared to truth (middle), and relative error between objective functions at each iteration (right) for the two parameter blind deconvolution setup.}
    %%\label{fig:enter-label}
\end{figure}


\begin{figure}[ht!]
    \centering
    \begin{subfigure}{.24\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/2/BD_objfn_opt_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.44\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/2/params_BD_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.22\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/2/BDFresults_yf_n32.png}
    \end{subfigure}   
    
    \caption{MM: Optimization iteration history using 2 inner iterations visualized on the objective function (left), individual parameters compared to truth (middle), and final reconstruction (right) for the two parameter blind deconvolution setup.}
    \label{fig:BD_MM2}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{.24\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/5/BD_objfn_opt_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.44\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/5/params_BD_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.22\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/5/BDFresults_yf_n32.png}
    \end{subfigure}   
    
    \caption{MM: Optimization iteration history using 5 inner iterations visualized on the objective function (left), individual parameters compared to truth (middle), and final reconstruction (right) for the two parameter blind deconvolution setup.}
    \label{fig:BD_MM5}
\end{figure}

\begin{figure}[ht!]
    \centering
    \begin{subfigure}{.24\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/10/BD_objfn_opt_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.44\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/10/params_BD_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.22\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/10/BDFresults_yf_n32.png}
    \end{subfigure}   
    
    \caption{MM: Optimization iteration history using 10 inner iterations visualized on the objective function (left), individual parameters compared to truth (middle), and final reconstruction (right) for the two parameter blind deconvolution setup.}
    \label{fig:BD_MM10}
\end{figure}

\begin{figure}[ht!]
    \centering
    \begin{subfigure}{.24\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/15/BD_objfn_opt_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.44\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/15/params_BD_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.22\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/MM/15/BDFresults_yf_n32.png}
    \end{subfigure}   
    
    \caption{MM: Optimization iteration history using 15 inner iterations visualized on the objective function (left), individual parameters compared to truth (middle), and final reconstruction (right) for the two parameter blind deconvolution setup.}
    \label{fig:BD_MM15}
\end{figure}

\begin{figure}[ht!]
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=0.3\textwidth]{SI/2/SI_objfuns.png} 
        & \includegraphics[width=0.3\textwidth]{SI/5/SI_objfuns.png} \\
        (a) & (b) \\
        \includegraphics[width=0.3\textwidth]{SI/10/SI_objfuns.png} 
        & \includegraphics[width=0.3\textwidth]{SI/25/SI_objfuns.png} 
        \\
        (c) & (d)
    \end{tabular}
    \caption{The full objective function evaluated at each iteration using SAA and MM with 2 (a), 5 (b), 10 (c), and 15 (d) maximum inner iterations for the two parameter blind deconvolution problem.}
    \label{fig:BD_objplots}
\end{figure}

\begin{figure}
\begin{minipage}{.6\textwidth}
\centering
\begin{tabular}{|c|c|c|c|}
    \cline{2-4}
    \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{SAA} \\ \cline{2-4} 
    \multicolumn{1}{c|}{} & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} \\ 
    \multicolumn{1}{c|}{} & Iter. & Evals. &  \\ \cline{2-4}
    \multicolumn{1}{c|}{} & 11 & 29 & 143 \\
    \cline{2-4} 
    \multicolumn{4}{c}{} \\
    \hline
    \multicolumn{4}{|c|}{MM} \\ \hline
    Maximum & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} \\
    Inner Iter. & Iter. & Evals. &  \\ \hline
    2 & 15 & 133 & 250 \\
    5 & 35 & 230 &  432 \\
    10 & 44 & 298 & 553 \\
    15 & 48 & 309 & 559 \\ \hline
\end{tabular}
\captionof{table}{Total iterations, function evaluations, and runtime for SAA and MM approach in the blind deconvolution problem.}
\end{minipage}
\hfill
\begin{minipage}{.37\textwidth}
\centering
\includegraphics[width=1\textwidth]{BDresults/BD_mmIterAll_n32.png}
\captionof{figure}{Number of inner iterations completed at each outer iteration for various maximum inner iterations for blind deconvolution problem.}
\end{minipage}
\end{figure}

%The SAA method is run using a range of Monte Carlo samples between 8 and 200 

We then used the SAA objective function with 100 Monte Carlo samples within an interior-point method with an initial guess of $\bfy_0=[1,2]\t$. The optimizer took 11 iterations to converge at $\bfy_f = [1.451,1.14]\t$.
The true and observed images, with a $1\%$ noise level, are in Figure \ref{fig:BD_im} along with reconstructions at $\bfy_t$, $\bfy_0$, and $\bfy_f$. Table \ref{tab:BD_times} provides the timings of both the SAA approach and the MM approach with varying maximum inner iterations.

% We then implement an interior-point method with an initial guess of $\bfy = []\t$ and 100 Monte Carlo samples. In the bottom panel of Figure \ref{fig:BD} we plot the history of the relative error (left), visualization of iterations across the optimization routine (middle) and the reconstruction at the final iteration (right). 
% The optimizer took () iterations for convergence at $\bfy = []\t$.

We then test the SAA method to estimate all parameters $\bfy_c = [l_1,l_2,l_3]\t$ keeping the fixed $\lambda=1/200$ and $\sigma = 5.55e-06$. For this setup, $\bfy_t = [1.016,-0.127,0.707]\t$ and the same optimization scheme was used with an initial guess of $\bfy_0 = [2,0,1]\t$. The optimizer took 11 iterations to converge at $\bfy_f = [1.028,-0.064,0.916]\t$. The true and observed images, with a $1\%$ noise level, are in Figure \ref{fig:BD3_im} along with reconstructions at $\bfy_t$, $\bfy_0$, and $\bfy_f$, model parameters.


\begin{figure}
\centering
\begin{tabular}{cc|ccc}
    \multirow{2}{*}{True} & \multirow{2}{*}{Observed} & \multicolumn{3}{c}{Reconstructions} \\
    & & $\bfy_t$ & $\bfy_0$ & $\bfy_f$ \\
    \includegraphics[width=.165\textwidth]{BDresults/BD3/BD3_true_n32.png} & 
    \includegraphics[width=.165\textwidth]{BDresults/BD3/BD3_blur_n32.png} & 
    \includegraphics[width=.165\textwidth]{BDresults/BD3/BD3Fresults_yt_n32_Ireg_l.png} & 
    \includegraphics[width=.165\textwidth]{BDresults/BD3/BD3Fresults_y0_n32_Ireg_l.png} & 
    \includegraphics[width=.165\textwidth]{BDresults/BD3/BD3Fresults_yf_n32_Ireg_l.png}
    
\end{tabular}
\caption{The true and observed images and reconstructions at $\bfy_t$, $\bfy_0$, and $\bfy_f$ for the three parameter blind deconvolution setup.}
\label{fig:BD3_im}
\end{figure}

\begin{figure}
    \centering
    
    \begin{subfigure}{.72\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/BD3/params_BD3_n32_Ireg_l.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.24\textwidth}
    \centering
        \includegraphics[width=1\linewidth]{BDresults/BD3/BD3_opt_error_n32_Ireg_l.png}
    \end{subfigure}
    
    \caption{SAA: Optimization iteration history as individual parameters compared to truth (left) and relative error between objective functions at each iteration (right) for the three parameter blind deconvolution setup.}
    %\label{fig:enter-label}
\end{figure}

% \begin{figure}
%     \centering

%     \begin{subfigure}{.74\textwidth}
%     \centering
%         \includegraphics[width=1\linewidth]{BDresults/MM/BD2_2/params_BD_n32.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.24\textwidth}
%     \centering
%         \includegraphics[width=.95\linewidth]{BDresults/MM/BD2_2/BDFresults_yf_n32.png}
%     \end{subfigure}
    
%     \begin{subfigure}{1\textwidth}
%     \centering
%         \includegraphics[width=.35\linewidth]{BDresults/MM/BD2_2/BD_objfn_comb_n32.png}
%     \end{subfigure}
    
    
%     \caption{MM with 2 inner iterations: Individual parameters compared to truth at each iteration (top left), final reconstruction (top right), and a comparison of the full objective function value using MM and SAA (bottom) for the three parameter blind deconvolution setup.}
%     %\label{fig:enter-label}
% \end{figure}

% \begin{figure}
%     \centering

%     \begin{subfigure}{.74\textwidth}
%     \centering
%         \includegraphics[width=1\linewidth]{BDresults/MM/BD2_3/params_BD_n32.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.24\textwidth}
%     \centering
%         \includegraphics[width=.95\linewidth]{BDresults/MM/BD2_3/BDFresults_yf_n32.png}
%     \end{subfigure}
    
%     \begin{subfigure}{1\textwidth}
%     \centering
%         \includegraphics[width=.35\linewidth]{BDresults/MM/BD2_3/BD_objfn_comb_n32.png}
%     \end{subfigure}
    
    
%     \caption{MM with 3 inner iterations: Individual parameters compared to truth at each iteration (top left), final reconstruction (top right), and a comparison of the full objective function value using MM and SAA (bottom) for the three parameter blind deconvolution setup.}
%     %\label{fig:enter-label}
% \end{figure}

% \subsubsection{Hierarchical Bayesian Inverse Problem}

% Now we change the problem so that the hyperparameters $\bftheta$ are unknown.

% \begin{figure}[H]
% \begin{tabular}{c c}
%     \includegraphics[width=.75\textwidth]{BDresults/BD2/params_BD2_n32_Ireg_v2.png} & \includegraphics[width=.25\textwidth]{BDresults/BD2/BD2Fresults_n32_Ireg_v2.png}  \\
% \end{tabular}
% \end{figure}

% \subsubsection{Linear Bayesian Inverse Problem}

% To verify that the optimization procedure correctly estimates the hyperparameters $\bftheta$, we fix $\bfA = \bfA(\bfy_t)$. Now we have a linear Bayesian inverse problem where the posterior distribution is given by $\pi(\bfx\mid \bftheta)$ and the marginal posterior distribution we wish to maximize is $\pi(\bftheta\mid\bfb)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> intro.tex <==
% \begin{itemize}
%     \item General inverse problem and examples
%     \item Nonlinear separable and examples
%     \item Bayesian approach
%     \item Parameter estimation - stochastic approach
%     \item Trace estimation - connections to SAA paper and then explore using other trace estimators (funNystrom)

%     \item Contributions and related work?

%     \item Outline of paper
    
% \end{itemize}

For large-scale inverse problems, parameter estimation remains a challenging task. Even in the case of linear inverse problems, many methods require function evaluations that are computationally infeasible. Especially in the case of separable nonlinear inverse problems where the model parameters that define the forward model are also unknown.

In this work, we consider Bayesian inverse problems where the unknown inverse parameters, model parameters, and observations are modeled as random variables. Moreover, we focus on problems where the forward model is nonlinear but separable.  That is, we consider large-scale inverse problems of the form
\begin{equation}
\label{eq:separable}
\bfb = \bfA(\bfy) \bfx + \bfe
\end{equation}
where $\bfb \in \bbR^m$ contains the observed measurement data vector, $\bfA(\cdot): \bbR^p \to \bbR^{m \times n}$ maps unknown model parameters $\bfy \in \bbR^p$ to a large, severely ill-conditioned matrix, $\bfx \in \bbR^n$ contains unknown inverse parameters, and $\bfe \in \bbR^m$ represents noise or error in the data.  
In many scenarios, it is assumed that $\bfy$ is known or can be well approximated.  However, there are many examples where separable nonlinear models arise including super-resolution, motion correction, and uncertain view angles \cite{chung2010efficient,espanol2023variable,cornelio2014constrained}.  Most works have focused on exploiting the separable structure to solve separable nonlienar least-squares problems efficiently, e.g., using variable projection approaches and comparing to alternating optimization and coupled approaches \cite{golub2003separable,ruhe1980algorithms,o2013variable,chung2010efficient}. Other works construct methods for estimating the model parameters... \cite{}.


Here, the goal is to construct a distribution of possible solutions given by the posterior probability distribution $\pi(\bfx,\bfy\mid \bfb)$ that, by Bayes' law, combines information from the measurements in the likelihood function and knowledge about the unknown inverse parameters and model parameters defined by the prior. We consider two cases. One in which the hyperparameters that define the likelihood function and prior of the unknown parameters are fixed and one where they are modeled as random variables and so must be approximated. The latter case requires a hierarchical Bayesian approach, meaning that the prior distribution of the unknown inverse parameters depends jointly on the hyperparameters. There are many challenges for both linear and nonlinear inverse problems, $\pi(\bfx,\bfy\mid \bfb)$ may not be Gaussian, and the number of unknowns may be large, making typical approaches (e.g., Markov Chain Monte Carlo methods) computationally infeasible.

However, there are methods that estimate only the model parameters and hyperparameters by marginalizing the unknown parameters from the joint posterior distribution to obtain the marginal posterior distribution $\pi(\bfy \mid \bfb)$, and compute a maximum a posteriori (MAP) estimate.
Similar work has been done in the case where the posterior distribution is fully Gaussian \cite{Hall-Hooper_Saibaba_Chung_Miller_2024} and where the forward operator is fixed but the posterior distribution may be non-Gaussian \cite{chung2024efficient}. In this paper, we use the approach in \cite{chung2024efficient} where a sample average approximation (SAA) is used to compute the MAP estimate. However, we extend the idea to problems where the forward operator depends nonlinearly on unknown model parameters.

The paper makes the following contributions: (1) we extend the SAA method for marginal posterior distributions to separable nonlinear inverse problems; (2) implementing trace estimation (might change depending on if we go the route of changing the trace estimator); (3) we demonstrate our method on blind deconvolution and super-resolution problems.

In Section \ref{sec:sepNonLin} we provide an overview of separable nonlinear Bayesian inverse problems and the resulting optimization problem for parameter estimation. Then in Section \ref{sec:optimization} we describe two computational approaches to efficiently perform parameter estimation.   Numerical results are provided in Section \ref{sec:NumEx} followed by conclusions and discussion in Section \ref{sec:ConcDisc}.

% model the intro off sep non lin sampling
% add in the problem, move the first chunk up of 2 into intro

%abstract
%1.context
%2. motivation
%3. approach
%4. contributions
%5. applications and results

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> old/old.tex <==
\begin{figure}[H]
    \centering
    \begin{subfigure}{.45\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{mc_nonlin_results/params_BD_n32_Q.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.45\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{mc_nonlin_results/params_BD_n32_I.png}
    \end{subfigure}
    \caption{Blind Deconvolution: Parameters at each iteration for $\bfQ_x$ matern (left) and $\bfQ_x=\bfI$ (right)}
    \label{fig:BDparam_SAA}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}{.9\linewidth}
        \includegraphics[width=1\linewidth]{mc_nonlin_results/BDresults_n32_Q.png}
        \caption{$\bfQ_x$ matern}
    \end{subfigure}
    \begin{subfigure}{.9\linewidth}
        \includegraphics[width=1\linewidth]{mc_nonlin_results/BDresults_n32_I.png}
        \caption{$\bfQ_x = \bfI$}
    \end{subfigure}
    \caption{Blind Deconvolution reconstructions for different $\bfQ_x$}
    \label{fig:BD_recon}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \begin{subfigure}{.9\textwidth}
%         \centering
%         \includegraphics[width=.89\textwidth]{mc_nonlin_results/BDresults_n32_Q.png}
%         \caption{Backslash}
%     \end{subfigure}
%     \begin{subfigure}{.9\textwidth}
%         \centering
%         \includegraphics[width=.9\textwidth]{mc_nonlin_results/HyBR_BD_n32_Q.png}
%         \caption{genHyBR without solver (top row) and genHyBR with Tikhonov solver (bottom row)}
%     \end{subfigure}
%     \caption{Blind Deconvolution $\bfQ_x$ matern}
%     \label{fig:BD_Q}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \begin{subfigure}{.9\textwidth}
%         \centering
%         \includegraphics[width=.89\textwidth]{mc_nonlin_results/BDresults_n32_I.png}
%         \caption{Backslash}
%     \end{subfigure}
%     \begin{subfigure}{.9\textwidth}
%         \centering
%         \includegraphics[width=.9\textwidth]{mc_nonlin_results/HyBR_BD_n32_I.png}
%         \caption{}
%     \end{subfigure}
%     \caption{Blind Deconvolution $\bfQ_x=\bfI$}
%     \label{fig:BD_I}
% \end{figure}

\begin{figure}[H]
    \begin{subfigure}{.4\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{mc_nonlin_results/params_BD_n32.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.57\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{mc_nonlin_results/GN_BD_n32.png}
    \end{subfigure}
    
    \caption{Blind Deconvolution. Gauss-Newton Results}
    \label{fig:BD_GN}
\end{figure}

%%%%%% Resp
\section{Respirometry}

\begin{figure}[H]
\centering
\begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{mc_nonlin_results/Resp_F_error.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\textwidth}
\centering
    \includegraphics[width=.8\textwidth]{mc_nonlin_results/Resp_G_error.png}
\end{subfigure}

\caption{Respirometry with initial guess: Relative error of the overall objective function (left) and relative error of gradient (right)}
\label{fig:Resp0}
\end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{mc_nonlin_results/Resp_F_errorTRUE.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\textwidth}
\centering
    \includegraphics[width=.8\textwidth]{mc_nonlin_results/Resp_G_errorTRUE.png}
\end{subfigure}

\caption{Respirometry with True Params: Relative error of the overall objective function (left) and relative error of gradient (right)}
\label{fig:RespT}
\end{figure}

Using an interior point method with $100$ iterations, and $100$ Monte Carlo samples, the signals were reconstructed from two different initial guesses. The first in Figure \ref{fig:RespRecon0} corresponds to an initial guess of all ones while Figure \ref{fig:RespReconG} corresponds to an initial guess based on the gamma function. For both, reconstructions from the initial guess are on the left while reconstructions after optimizing are on the right.

\begin{figure}[H]
\centering
\begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{mc_nonlin_results/Respyones_recon_0.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\textwidth}
\centering
    \includegraphics[width=1\textwidth]{mc_nonlin_results/Respyones_recon_f.png}
\end{subfigure}

\caption{Respirometry reconstructions with $y_0$ of ones (left) and reconstruction after 100 iterations (right)}
\label{fig:RespRecon0}
\end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{mc_nonlin_results/Respygamma_recon_0.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\textwidth}
\centering
    \includegraphics[width=1\textwidth]{mc_nonlin_results/Respygamma_recon_f.png}
\end{subfigure}

\caption{Respirometry reconstructions with gamma function $y_0$ (left) and reconstruction after 100 iterations (right)}
\label{fig:RespReconG}
\end{figure}

%%%%%%% BD figures for different Qx
\begin{figure}[H]
    \centering
    \begin{subfigure}{.45\textwidth}
        \includegraphics[width=.85\linewidth]{BDresults/BD_objfn_opt_n32_Ireg.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.45\textwidth}
        \includegraphics[width=.85\linewidth]{BDresults/BDFresults_n32_Ireg.png}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{.3\textwidth}
    %     \includegraphics[width=1\linewidth]{}
    % \end{subfigure}
    \caption{$\bfQ_x = \bfI$ with $\lambda=0.0005$: Iteration history plotted on the objective function (left) and reconstruction at final iteration (right)}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}{.45\textwidth}
        \includegraphics[width=.85\linewidth]{BDresults/BD_objfn_opt_n32_Q.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.45\textwidth}
        \includegraphics[width=.85\linewidth]{BDresults/BDFresults_n32_Q.png}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{.3\textwidth}
    %     \includegraphics[width=1\linewidth]{}
    % \end{subfigure}
    \caption{$\bfQ_x$ matern kernel with $\lambda=1$: Iteration history plotted on the objective function (left) and reconstruction at final iteration (right)}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}{.45\textwidth}
        \includegraphics[width=.85\linewidth]{BDresults/BD_objfn_opt_n32_Qreg.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.45\textwidth}
        \includegraphics[width=.85\linewidth]{BDresults/BDFresults_n32_Qreg.png}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{.3\textwidth}
    %     \includegraphics[width=1\linewidth]{}
    % \end{subfigure}
    \caption{$\bfQ_x$ matern kernel with $\lambda=0.0005$: Iteration history plotted on the objective function (left) and reconstruction at final iteration (right)}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{c c c c}
     \multicolumn{2}{c}{$\bfy_0$} &\multicolumn{2}{c}{ $\bfy_f$} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n64_k8_I_RI2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n64_k8_I_RI2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n64_k8_I_RI2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n64_k8_I_RI2.png} \\ 
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n64_k8_Q_RI2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n64_k8_Q_RI2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n64_k8_Q_RI2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n64_k8_Q_RI2.png} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n64_k8_I_RK2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n64_k8_I_RK2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n64_k8_I_RK2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n64_k8_I_RK2.png} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n64_k8_Q_RK2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n64_k8_Q_RK2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n64_k8_Q_RK2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n64_k8_Q_RK2.png}
\end{tabular}
\caption{SR 64x64 reconstructions for $\bfQ=\bfI$ and $\bfR=\bfI$; $\bfQ$ matern and $\bfR=\bfI$; $\bfQ=\bfI$ and $\bfR=\sigma\bfI$; and $\bfQ$ matern and $\bfR=\sigma\bfI$}
\label{fig:SRI}
\end{figure}

\begin{figure}
    \centering
    \begin{tabular}{c | c c c}
         True & Mat\'ern & $\bfQ_x = \lambda\bfI$ & 
         $\bfR=\bfI$, $\bfQ_x = \lambda\bfI$\\
        \includegraphics[width=.22\textwidth]{SRresults/SRresults_true.png}  
        & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yt_n32_Qreg_2.png} 
        & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yt_n32_Ireg_2.png} 
        & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yt_GN_k8.png} 
    \end{tabular}
    \caption{SR: From left to right, true image, reconstructions at $\bfy_t$ using Mat\'ern kernel, $\bfQ_x=\lambda\bfI$, and $\bfR=\bfI$, $\bfQ_x=\lambda\bfI$}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{c c c c}
      \multicolumn{2}{c}{$\bfy_0$} &\multicolumn{2}{c}{ $\bfy_f$} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n32_Qreg_2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n32_Qreg_2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n32_Qreg_2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n32_Qreg_2.png} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n32_Qreg.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n32_Qreg.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n32_Qreg.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n32_Qreg.png} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n32_Qreg_3.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n32_Qreg_3.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n32_Qreg_3.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n32_Qreg_3.png}
\end{tabular}
\caption{SR reconstructions and parameters at initial and final iterations using Mat\'ern kernel $\bfQ_x$ with scaled $\bfy_0$ and bound of $[-.2,.2]$ (top row), unscaled $\bfy_0$ and bound of $[-.7,.7]$ (middle row), and shifted $\bfy_0$ and bound of $[-.2,.2]$ (bottom row).}
\label{fig:SRmater}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{c c c c}
     \multicolumn{2}{c}{$\bfy_0$} &\multicolumn{2}{c}{ $\bfy_f$} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n32_Ireg_2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n32_Ireg_2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n32_Ireg_2.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n32_Ireg_2.png} \\ 
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n32_Ireg.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n32_Ireg.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n32_Ireg.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n32_Ireg.png} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_n32_Ireg_3.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_n32_Ireg_3.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_n32_Ireg_3.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_n32_Ireg_3.png}
\end{tabular}
\caption{SR reconstructions and parameters at initial and final iterations using $\bfQ_x=\lambda\bfI$ with scaled $\bfy_0$ and bound of $[-.2,.2]$ (top row), unscaled $\bfy_0$ and bound of $[-.7,.7]$ (middle row), and shifted $\bfy_0$ and bound of $[-.2,.2]$ (bottom row).}
\label{fig:SRI}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{c c c c}
     \multicolumn{2}{c}{$\bfy_0$} &\multicolumn{2}{c}{ $\bfy_f$} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults_y0_GN_k8.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_y0_SR_GN_k8.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults_yf_GN_k8.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params_yf_SR_GN_k8.png} \\
     \includegraphics[width=.22\textwidth]{SRresults/SRresults2_y0_GN_k8.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params2_y0_SR_GN_k8.png}
     & \includegraphics[width=.22\textwidth]{SRresults/SRresults2_yf_GN_k8.png}
     & \includegraphics[width=.22\textwidth]{SRresults/params2_yf_SR_GN_k8.png}
\end{tabular}
\caption{SR reconstructions and parameters at initial and final iterations using Gauss-Newton with $\bfQ_x=\lambda\bfI$ for unscaled $\bfy_0$ (top row) and scaled $\bfy_0$ (bottom row).}
\label{fig:SRGN}
\end{figure}


%%%%%%%% s,r setup for BD
We assume a Gaussian blur where the PSF, centered at $(k,l)$, has the form
\begin{align}
    p_{ij} &= \exp\left( -\frac{1}{2}\begin{bmatrix} i-k \\ j-l \end{bmatrix}\t \begin{bmatrix} s_1^2 & r^2 \\ r^2 & s_2^2 \end{bmatrix}^{-1} \begin{bmatrix} i-k \\ j-l \end{bmatrix}\right)  \label{eq:PSF} \\
    &= \exp\left(\frac{-(i-k)^2s_2^2-(j-l)^2s_1^2+2(i-k)(j-l)r^2}{2s_1^2s_2^2-2r^4}\right) \notag
\end{align}
% \begin{align*}
%     p_{ij} &= \exp\left( -\frac{1}{2}\begin{bmatrix} i-k \\ j-l \end{bmatrix}\t \begin{bmatrix} s_1^2 & 0 \\ 0 & s_2^2 \end{bmatrix}^{-1} \begin{bmatrix} i-k \\ j-l \end{bmatrix}\right) \\
%     &= \exp\left(-\frac{(i-k)^2}{2s_1^2}-\frac{(j-l)^2}{2s_2^2}\right)
% `\end{align*}
where the parameters $s_1$ and $s_2$ determine the spread and $r$ determines the rotation of the PSF. Let
\begin{equation*}
    \bfy = \begin{bmatrix}
        s_1 \\ s_2 \\ r
    \end{bmatrix}
\end{equation*}
and $\bfA(\bfy)$ be the Gaussian PSF with parameters $\bfy$.

\begin{figure}[H]
    \centering
    \begin{tabular}{c|ccc}
        $\scriptstyle\mc{F}(\bfy)$ & $\scriptstyle\frac12\logdet\Psi(\bfy)$ & $\scriptstyle\frac12 \|\bfA(\bfy) \bfmu_x - \bfb\|_{\bfPsi(\bfy)^{-1}}^2$ &  $\scriptstyle-\log\pi_{y}(\bfy)$ \\
        \includegraphics[width=.22\textwidth]{BDresults/BD_full_objfn_32_Ireg.png} &
        \includegraphics[width=.22\textwidth]{BDresults/BD_full_objfnF1_32_Ireg.png} &
        \includegraphics[width=.22\textwidth]{BDresults/BD_full_objfnF2_32_Ireg.png} &
        \includegraphics[width=.22\textwidth]{BDresults/BD_full_objfnF3_32_Ireg.png}
    \end{tabular}
        \caption{Full objective function over the grid $[0.25,2.5]\times [0.25,2.5]$.}
        \label{fig:objFun}
\end{figure}

\begin{figure}[H]
\centering

\begin{subfigure}{1\textwidth}
    \centering
    \includegraphics[width=.7\textwidth]{BDresults/params_BD_n32_Ireg.png}
    \caption{}
\end{subfigure}

\begin{subfigure}{0.3\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{BDresults/BD_F_error_n32_Ireg.png}
    \caption{}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
\centering
    \includegraphics[width=1\textwidth]{BDresults/BD_objfn_opt_n32_Ireg.png}
    \caption{}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
\centering
    \includegraphics[width=1\textwidth]{BDresults/BDFresults_yf_n32_Ireg.png}
    \caption{}
\end{subfigure}

\caption{Relative error of the overall objective function at varying Monte Carlo samples (a) and each iteration (b), the visualization of iterations (c) and reconstruction at the final iteration (d)}
\label{fig:BD_s}
    
\end{figure}

%%% matrix vs matvec
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    & $\bfA$ Matvecs & $\bfQ$ Matvecs & Time & Rel. Error 
    \\ \hline
    funMat & 11,413,240 & 5,689,537 &$3.37\times10^3$ & 0.228 \\ \hline
    Full Matrix & 40,918,776 & 20,397,492 & $3.56\times10^3$ & 0.194 
    \\ \hline
    \end{tabular}
    \caption{MM-SAA using projected gradient and finite difference with 150 inner iterations where $\bfA$ is a full matrix and a funMat}
    \begin{tabular}{c c }
    funMat & Full Matrix \\
    \includegraphics[width=.20\textwidth]{SRresults/matvec/150/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.20\textwidth]{SRresults/matrix/150/SRresults_yf_n128_k8.png} \\
    \includegraphics[width=.17\textwidth]{SRresults/matvec/150/params_yf_SR_n128_k8.png}  
    & \includegraphics[width=.17\textwidth]{SRresults/matrix/150/params_yf_SR_n128_k8.png} 
    \end{tabular}
\end{table}


%%%% table for SR - SAA and MM approach original (SAA no finite diff and MM projected gradient with finite difference)
\begin{figure}
\begin{minipage}{.67\textwidth}
\centering
\centering
\begin{tabular}{|c|c|c|c|c|}
    \cline{2-5}
    \multicolumn{1}{c|}{} & \multicolumn{4}{c|}{SAA} \\ \cline{2-5} 
    \multicolumn{1}{c|}{} & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} & Rel. \\ 
    \multicolumn{1}{c|}{} & Iter. & Evals. & &Error \\ \cline{2-5}
    \multicolumn{1}{c|}{} & 130 & 556 & $3.64\times 10^3$ & 0.196 \\
    \cline{2-5} 
    \multicolumn{5}{c}{} \\
    \hline
    % \multicolumn{5}{|c|}{MM-SAA} \\ \hline
    % Maximum & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} & Rel. \\
    % Inner Iter. & Iter. & Evals. & & Error \\ \hline
    % 2 & 1,000 & 9,414 & $5.13 \times 10^4$& \\
    % 50 & 1,176 & 5,376 & $2.97 \times 10^4$& \\
    % 100 & 615 & 2,730 & $1.46\times 10^4$ &\\
    % 150 & 228 & 1,032 & $5.59\times 10^3$& \\
    % 200 & 203 & 909 & $4.93\times 10^3$ &\\ \hline
    % \multicolumn{5}{|c|}{MM-SAA (Projected Gradient)} \\ \hline
    % Maximum & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} & Rel. \\
    % Inner Iter. & Iter. & Evals. & & Error \\ \hline
    % 50 & & &  & \\
    % 100 & & &  & \\
    % 150 &  & &  & 
    % \\ \hline 
    % \multicolumn{5}{c}{} \\
    % \hline
    \multicolumn{5}{|c|}{MM-SAA (Projected Gradient w/ Finite Diff.)} \\ \hline
    Maximum & Total & Total Fn. & \multirow{2}{*}{Runtime (s)} & Rel. \\
    Inner Iter. & Iter. & Evals. & & Error \\ \hline
    50 & 2,028 & & $4.94\times 10^3$  & 0.191 \\
    100 & 2,612 & &$6.19\times 10^3$ & 0.190 \\
    150 & 1,222 & &$2.85\times 10^3$  & 0.197 \\
    200 & 1,315 & & $3.07\times 10^3$ & 0.196
    \\ \hline
\end{tabular}
\captionof{table}{Total iterations, function evaluations, and runtime for SAA and MM approach in the $128\times 128$ super resolution problem. The relative error of the reconstruction at $\bfy_t$ is 0.178.}
\end{minipage}
\hfill
\begin{minipage}{.28\textwidth}
\centering
\includegraphics[width=1\textwidth]{SRresults/FD/SR_mmIterAll_n128.png}
\captionof{figure}{Number of inner iterations completed at each outer iteration for various maximum inner iterations for the $128\times 128$ super resolution problem.}
\end{minipage}
\end{figure}

%%%% objective function evaluations for mm-saa SI
\begin{figure}
    \centering
    \begin{tabular}{c c c}
        \includegraphics[width=.3\textwidth]{SI/SI_big/SIobj_SAA.png} & \includegraphics[width=.3\textwidth]{SI/SI_big/2/SIobj_MM.png} & \includegraphics[width=.3\textwidth]{SI/SI_big/5/SIobj_MM.png} \\
        \includegraphics[width=.3\textwidth]{SI/SI_big/10/SIobj_MM.png} & \includegraphics[width=.3\textwidth]{SI/SI_big/15/SIobj_MM.png} & \includegraphics[width=.3\textwidth]{SI/SI_big/20/SIobj_MM.png}
    \end{tabular}
    \caption{The full objective function Evaluations at each iteration for the Seismic Inversion problem}
\end{figure}

%%%% figures for MM-SAA projected gradient with finite difference for various inner iterations
\begin{figure}
\begin{tabular}{|c c c|}
    \hline
    \multicolumn{3}{|c|}{MM-SAA} 
    \\ \hline %\hline
    \multicolumn{3}{|c|}{$128\times128$: $\lambda=25$ and $\sigma=0.13$} 
    \\ \hline
    $\bfy_t$ &  \multicolumn{2}{c|}{$\bfy_0$} 
    \\
    \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_yt_n128_k8.png}
    & \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_y0_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/SR/params_y0_SR_n128_k8.png} 
    \\ \hline
    Maximum & \multicolumn{2}{c|}{$\bfy_f$} \\
    Inner Iteration & &
    \\
    2 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/2/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/2/params_yf_SR_n128_k8.png}
    \\
    50 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/50/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/50/params_yf_SR_n128_k8.png}
    \\
    100 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/100/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/100/params_yf_SR_n128_k8.png}
    \\
    150 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/150/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/150/params_yf_SR_n128_k8.png}
    \\
    200 
    & \includegraphics[width=.20\textwidth]{SRresults/MM/300/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/MM/300/params_yf_SR_n128_k8.png}
    \\ \hline
\end{tabular}
\caption{SR $128\times 128$ reconstructions and parameters at $\bfy_t$, $\bfy_0$, and $\bfy_f$ for MM approach using varying maximum inner iterations. (int point)}
%\label{fig:placeholder}
\end{figure}


%%%%%% proj grad dec with finite difference
\begin{figure}
\centering
\begin{tabular}{|c c c|}
    \hline
    \multicolumn{3}{|c|}{MM-SAA: Projected Gradient with Finite Difference} 
    \\ \hline %\hline
    \multicolumn{3}{|c|}{$128\times128$: $\lambda=25$ and $\sigma=0.13$} 
    \\ \hline
    $\bfy_t$ &  \multicolumn{2}{c|}{$\bfy_0$} 
    \\
    \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_yt_n128_k8.png}
    & \includegraphics[width=.20\textwidth]{SRresults/SR/SRresults_y0_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/SR/params_y0_SR_n128_k8.png} 
    \\ \hline
    Maximum & \multicolumn{2}{c|}{$\bfy_f$} \\
    Inner Iteration & &
    \\
    50 
    & \includegraphics[width=.20\textwidth]{SRresults/FD/50/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/FD/50/params_yf_SR_n128_k8.png}
    \\
    100 
    & \includegraphics[width=.20\textwidth]{SRresults/FD/100/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/FD/100/params_yf_SR_n128_k8.png}
    \\
    150 
    & \includegraphics[width=.20\textwidth]{SRresults/FD/150/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/FD/150/params_yf_SR_n128_k8.png}
    \\
    200 
    & \includegraphics[width=.20\textwidth]{SRresults/FD/200/SRresults_yf_n128_k8.png} 
    & \includegraphics[width=.17\textwidth]{SRresults/FD/200/params_yf_SR_n128_k8.png}
    \\ \hline
\end{tabular}
\caption{SR $128\times 128$ reconstructions and parameters at $\bfy_t$, $\bfy_0$, and $\bfy_f$ for MM approach with projected gradient using varying maximum inner iterations.}
%\label{fig:placeholder}
\end{figure}

\begin{figure}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{|c|cc|cc|}
    \hline
    & \multicolumn{2}{c|}{\textbf{Interior Point}} & \multicolumn{2}{c|}{\textbf{Projected Gradient}}
    \\ \hline
    \raisebox{24pt}{\textbf{SAA}} & \includegraphics[width=.19\textwidth]{SRresults/new/saa_int/SRresults_yf_n128.png}
     & 
     \includegraphics[width=.16\textwidth]{SRresults/new/saa_int/params_yf_SR_n128.png} & \includegraphics[width=.19\textwidth]{SRresults/new/saa_pgd/SRresults_yf_n128.png}
     & 
     \includegraphics[width=.16\textwidth]{SRresults/new/saa_pgd/params_yf_SR_n128.png} \\
    \raisebox{24pt}{\textbf{MM-SAA}} & \includegraphics[width=.19\textwidth]{SRresults/new/mm_int/SRresults_yf_n128_k8.png}
     & 
     \includegraphics[width=.16\textwidth]{SRresults/new/mm_int/params_yf_SR_n128_k8.png} & \includegraphics[width=.19\textwidth]{SRresults/new/mm_pgd/SRresults_yf_n128_k8.png}
     & 
     \includegraphics[width=.16\textwidth]{SRresults/new/mm_pgd/params_yf_SR_n128_k8.png}
     \\ \hline
\end{tabular}
\caption{Approximate Gradient - Elle: update new results}
\label{fig:SR_results}
\end{figure}
